Unsupervised HDR Imaging: What Can Be Learned from a Single 8-bit Video?

Recently, Deep Learning-based methods for inverse tone-mapping standard dynamic range (SDR) images to obtain high dynamic range (HDR) images have become very popular. These methods manage to fill over-exposed areas convincingly both in terms of details and dynamic range. Typically, these methods, to be effective, need to learn from large datasets and to transfer this knowledge to the network weights. In this work, we tackle this problem from a completely different perspective. What can we learn from a single SDR video? With the presented zero-shot approach, we show that, in many cases, a single SDR video is sufficient to be able to generate an HDR video of the same quality or better than other state-of-the-art methods.

==> results_scene.tex <==
%\begin{table}[ht]
% \centering
%\begin{tabular}{|l|lllll|}
%\hline
% \textbf{puPSNR} &  Eil & Santos & Our  & Exp & Endo \\
% \textbf{puSSIM} &  Our & Eil   & Santos & Exp & Endo \\
% \textbf{HDR-VDP} 2.2 &  Eil & Santos & Our & Exp & Endo \\
%\hline
% \end{tabular}
%\caption{\label{tab:comp:sr} Scene-referred comparisons for the results shown in Table \ref{tab:results:sr}. Methods are sorted by mean value. Color groupings show that there was no significant difference between those methods. for pairwise comparisons with Bonferroni corrections. The methods are: Santos (Santos et al.), Eil ( Elierstein et al.), Exp (Marnerides et al.), Endo (Endo et al.) and Our (the presented method).}
%\end{table}

\begin{table}
    \centering
    \small{
%    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{STU  dataset}\\
    \hline
    \textbf{Method} & \textbf{PU-PSNR} & \textbf{PU-SSIM} & \textbf{HDR-VDP3}\\
    \hline
OUR & 35.086358 &   \bluet{0.972743} &  9.7903  \\
SAN &  \bluet{36.628900}  & 0.971556 & \bluet{9.8943}\\
EIL &  \redt{38.622859}  &   \redt{0.974154} & \redt{9.9220} \\
EXP & 31.130048  &  0.912241 & 9.6348 \\    
DRT & 23.172132  & 0.463621  & 8.2215\\
    \hline
    \multicolumn{4}{|c|}{UBC  dataset}\\
    \hline
OUR & 41.247889  & 0.982170 & 9.9549\\
SAN &  \redt{44.851523}  &  \redt{0.987708}  & \redt{9.9897}\\
EIL & \bluet{43.414053}  &  \bluet{0.985220} & \bluet{9.9859}\\
EXP & 36.666005  &  0.934807&9.9426\\    
MRT & 27.883826  &   0.518727&8.9834\\
    \hline
    \multicolumn{4}{|c|}{COST  dataset}\\
    \hline
OUR & \redt{58.565082}  & 0.996284 & 9.9865\\
SAN & \bluet{53.618304}  &  \redt{0.997643} &  \redt{9.9944}  \\
EIL & 52.204955  &  \bluet{0.997031} &  \bluet{9.9933}\\
EXP & 50.338540  &  0.995216 & 9.9840\\    
MRT & 36.275900  &   0.973565 &  9.4751\\

    \hline
    \end{tabular}
  %  }
    }
    \caption{\small{This table reports the HDR-VDP3 (the maximum quality value is 10.0), PU-PSNR and PU-SSIM mean values for scene-referred videos. The red font color is for the best method, and the blue one is for the second-best one.}}
    \label{tab:results:sr}
\end{table}



%
%Further detail of the results distributions can be seen in the boxplots, one for each metric and type of video (i.e., scene-referred and display-referred), in Figure~\ref{fig:hdrvdp:boxplot} (HDR-VDP3), in Figure~\ref{fig:pupsnr:boxplot} (PU-PSNR), and in Figure~\ref{fig:pupsnr:boxplot} (PU-SSIM).

%Furthermore, Table \ref{tab:comp:dr} presents significant differences between the methods using pairwise comparisons with Bonferroni corrections. Color groupings denote a lack of significant differences between the methods. 
%EIL performs best overall, this is probably due to its updated focus on videos, with SAN performing well. Our method is in the top group for all metrics except HDR-VDP3, suggesting that it is largely competitive, which demonstrates good performance considering it is learning the mapping of the videos to HDR on the fly without prior knowledge.  

==> results_sig_asia.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{img/framework.png}
    \caption{\small{Overview of the framework. At training, a cyclical consistency loss is used to train both the down-exposure and up-exposure networks (\netup{} and \netdown{}). $\mathcal{L}_d$ is the down-exposure loss and $\mathcal{L}_u$ is the cyclical up-exposure loss. At inference time, the networks are then used sequentially to produce four additional exposures.}}
    \label{fig:framework}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{img/timings.pdf}
    \caption{\small{Timings for training a single epoch against input SDR video duration. These timings were measured on the 46 videos used in Section~\ref{sec:results:quantitative}.}}
    \label{fig:timings:epoch}
\end{figure}

\begin{table}
    \centering
    \small{
%    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|}
    \hline
    \textbf{Method} & \textbf{HDR-VDP 2.2} & \textbf{PU-PSNR} & \textbf{PU-SSIM}\\
    \hline
    OUR                 & 55.087522         &   36.217375           & \redt{0.975406}\\
    SAN       & \bluet{58.488099} &   \bluet{36.757138}   & 0.964260\\
    EIL    & \redt{58.983167}  &   \redt{38.244785}    & \bluet{0.967825}\\
    EXP   & 53.303279         &   31.064146           & 0.894365\\
    DRT         & 42.105403         &   24.075940           & 0.684500\\
    \hline
    \end{tabular}
  %  }
    }
    \caption{\small{This table reports the HDR-VDP 2.2, PU-PSNR and PU-SSIM mean values for 46 scene-referred videos. The red font color is for the best method, and the blue one is for the second-best one.}}
    \label{tab:results:sr}
\end{table}


\begin{table}
    \centering
    \small{
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|}
    \hline
    \textbf{Method} & \textbf{HDR-VDP 2.2} & \textbf{PU-PSNR} & \textbf{PU-SSIM}\\
    \hline
    OUR          & 57.740986         &   \bluet{33.905331}   & \redt{0.982263}\\
    SAN          & \bluet{61.293401} &   33.240828           & 0.977762\\
    EIL          & \redt{61.559705}  &   \redt{34.510490}   & \bluet{0.978264}\\
    EXP          & 54.876668         &   26.403320           & 0.903216\\
    DRT          & 44.076568         &   17.930416           & 0.674483\\
            \hline
    \end{tabular}
    }
    }
    \caption{\small{This table reports the HDR-VDP 2.2, PU-PSNR and PU-SSIM mean values for 46 display-referred videos. The red font color is for the best method, and the blue one is for the second-best one.}}
    \label{tab:results:dr}
\end{table}

\begin{table}[ht]
 \centering
 \small{
\begin{tabular}{|l|lllll|}
 \hline
  \textit{Scene-referred} & & & & & \\
  \textbf{PU-PSNR} &  EIL & SAN & OUR  & EXP & DRT \\
 \textbf{PU-SSIM} &  OUR & EIL   & SAN & EXP & DRT \\
 \textbf{HDR-VDP 2.2}  & EIL & SAN & OUR & EXP & DRT \\
\hline
  \textit{Display-referred} & & & & & \\
 \textbf{PU-PSNR} &  EIL & OUR & SAN  & EXP & DRT \\
 \textbf{PU-SSIM} &  OUR & EIL & SAN  & EXP & DRT \\
 \textbf{HDR-VDP 2.2} &  EIL & SAN  & OUR & EXP & DRT \\
\hline
 \end{tabular}
 }
\caption{\label{tab:comp:dr} Scene-referred comparisons (top) for the results shown in Table \ref{tab:results:sr} and display-referred comparisons (bottom) for the results shown in Table \ref{tab:results:dr}. Methods are sorted by mean value. Color groupings show that there was no significant difference between those methods for pairwise comparisons with Bonferroni corrections.} 
%The methods are: SAN (Santos et al.), EIL ( Eilerstein et al.), EXP (Marnerides et al.), DRT (Endo et al.) and OUR (the presented method). }
\end{table}



\begin{figure}
    \centering
    \includegraphics[width=0.48\linewidth]{img/psnr_sr.pdf}
    \includegraphics[width=0.48\linewidth]{img/psnr_dr.pdf}
    \caption{\small{Boxplots of PU-PSNR for 46 videos: On the left side, results for scene-referred videos. On the right side, results for display-referred videos.}}
    \label{fig:pupsnr:boxplot}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.48\linewidth]{img/SSIM_sr.pdf}
    \includegraphics[width=0.48\linewidth]{img/SSIM_dr.pdf}
    \caption{\small{Boxplots for PU-SSIM for 46 videos: On the left side, results for scene-referred videos. On the right side, results for display-referred videos.}}
    \label{fig:puSSIM:pusssim}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.48\linewidth]{img/vdp_sr.pdf}
    \includegraphics[width=0.48\linewidth]{img/vdp_dr.pdf}
    \caption{\small{Boxplots for HDRVDP 2.2 for 46 videos: On the left side, results for scene-referred videos. On the right side, results for display-referred videos.}}
    \label{fig:hdrvdp:boxplot}
\end{figure}
